Causal Analysis of Syntactic Agreement Mechanisms in Neural Language Models

Targeted syntactic evaluations have demonstrated the ability of language models to perform subject-verb agreement given difficult contexts. To elucidate the mechanisms by which the models accomplish this behavior, this study applies causal mediation analysis to pre-trained neural language models. We investigate the magnitude of models' preferences for grammatical inflections, as well as whether neurons process subject-verb agreement similarly across sentences with different syntactic structures. We uncover similarities and differences across architectures and model sizes -- notably, that larger models do not necessarily learn stronger preferences. We also observe two distinct mechanisms for producing subject-verb agreement depending on the syntactic structure of the input sentence. Finally, we find that language models rely on similar sets of neurons when given sentences with similar syntactic structure.

==> scrap.tex <==
% \subsection{Natural Direct Effect: How much of the observed effect flows outside of a particular neuron or attention head?}

% The natural direct effect (NDE) may be conceptualized as the complement of the natural indirect effect. The NDE measures the change in effect when $u$ is changed, but $\mathbf{z}$ is kept at the value it had before $u$ was changed:

% \begin{align}
%     \begin{split}
%         \overline{\text{NDE}}(\texttt{swap-subject, null};y,\mathbf{z}) = \\
%         \mathbb{E}_{u,v}\left[ \frac{y_{\texttt{swap-number},\mathbf{z}_{\texttt{null}}(u,v)}(u,v)}{y_\texttt{null}(u,v)} - 1 \right]
%     \end{split}
% \end{align}

% We generally expect this quantity to be much larger than indirect effects when $\mathbf{z}$ is a small part of the model, for the NDE measures how much the model without $\mathbf{z}$ contributes to the total effect. We do not focus on this quantity as much as indirect effects, as it gives us less specific information regarding which components are implicated in observed behaviors.

% \subsection{Attention Heads}

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{attention_indirect/distractor_effect_bars.pdf}
%    \caption{Total (TE), direct (NDE-all), and indirect effects (NIE-all and NIE-sum) for attention heads for the `across a distractor' structure. NIE-all (the indirect effect from simultaneously intervening on all attention heads) and NIE-sum (the indirect effect from summing independent and separate interventions on each attention head) are near zero and thus not visible.}
%    \label{fig:attn_effects}
%\end{figure}

%\begin{figure*}
%    \centering
%    \begin{minipage}{0.48\linewidth}
%    \includegraphics[width=\linewidth]{attention_indirect_zero/within_rc_singular_zero_gpt2_filtered.pdf}
%    \end{minipage}
%    \hfill
%    \begin{minipage}{0.48\linewidth}
%    \includegraphics[width=\linewidth]{attention_indirect_zero/plural_zero_gpt2_filtered.pdf}
%    \end{minipage}
%    \caption{Attention head indirect effects for GPT-2 Small under the \texttt{zero} intervention. We only present a subset of structures to demonstrate consistency of implicated attention heads across different kinds of structures; figures for all structures may be found in Appendix~\ref{app:attn}.}
%    \label{fig:attn_zero}
%\end{figure*}

% Trends are generally less clear for attention heads. Each structure appears to have completely different heads with significant indirect effects; even changing the number of the attractor has a large effect on which heads are implicated in observed behavior. See Appendix~\ref{app:attn}.

% Perhaps a reason for this is that most of the total effect does not flow through the attention heads. We find that the sum of the indirect effects across heads averaged across prompts is always near-zero (and is often small and negative), as is the indirect effect attained when intervening on all attention heads simultaneously. Meanwhile, the direct effect across heads is very large and captures most of the total effect. See Figure~\ref{fig:attn_effects}. This indicates that most of the total effect does not flow through the attention heads, but through other model components (e.g., word representations, neurons). Thus, perhaps what specific heads are displaying across structures is noise, rather than meaningful effects.

% To test whether attention is simply robust to the \texttt{swap-number} intervention, we define an alternate intervention \texttt{zero}: rather than swapping the number of the subject, we set a specific attention head $\mathbf{z}$'s value to $0$ and observe how this changes the effect on the unchanged prompt. This may be interpreted as the controlled direct effect, as defined in \citet{pearl2001direct}.


% For this intervention, trends are much more consistent across structures. Head 0-10 is always strongly implicated in behavior; since this is in the bottom layer, this indicates that much of attention's contribution to syntax is lexicalized. In other words, attention's contribution to subject-verb agreement may largely be based on which word embeddings are present in the input, rather than any compositional structural information that would be present in the upper layers.

% For all structures except where we have adverbial distractors, we see consistent positive indirect effects in the uppermost layers as well. No single attention head appears strongly implicated (though head 11-0 is always positive), but the layer effect is consistently positive and sometimes nears the magnitude of the layer effect of layer 0. This indicates that more abstract structural information is quite distributed across attention heads in the uppermost layers, but nonetheless may be present.


